Bounded Parikh Automata

The Parikh finite word automaton model (PA) was introduced and studied by Klaedtke and Ruess in 2003. Here, by means of related models, it is shown that the bounded languages recognized by PA are the same as those recognized by deterministic PA. Moreover, this class of languages is the class of bounded languages whose set of iterations is semilinear.

==> define.tex <==
%% Macros and other LaTeX definitions.

\makeatletter

\def\Tau{\text{\rm T}}
\def\calC{\mathcal{C}}
\def\monP{\mathcal{P}}
\def\mon{\mathcal{M}}
\def\up{\mathsf{Up}}
\def\low{\mathsf{Low}}
\def\eps{\varepsilon}
\def\mat{\mathcal{M}}
\def\iter{\mathsf{Iter}}
\def\bbn{\ensuremath{\mathbb{N}}\xspace}
\def\bbz{\ensuremath{\mathbb{Z}}\xspace}
\def\pkh{\ensuremath{\Phi}}
\def\nothmspace{\vspace{-4\p@}}
\def\func{\mathcal{F}}
\def\powerset{\mathcal{P}}
\def\st{\;|\;}
\def\apaths{\ensuremath{\mathsf{Run}}}
\def\Id{\mathit{Id}}
\def\KaR{Klaedtke and Rue\ss\xspace}
\def\proj{\Psi}
\def\pext{\tilde\Phi}
\def\@@one!#1,#2!{\mathbb{1}_{(\@ifempty{#2}{#1,\cdot}{\@ifempty{#1}{\cdot,#2}{#1,#2}})}}
\def\one#1{\@@one!#1!}
\def\zero{\mathbb{0}}
\def\orig{\mathsf{From}}
\def\dest{\mathsf{To}}
\def\restr#1{\!\!\upharpoonright_{#1}\,}

\def\und#1{\begingroup\setbox0=\hbox{$#1$}\leavevmode%
  \hbox to 0pt{\vrule depth 1.2pt height -.75pt width \wd0\hss}%
  #1\endgroup}

%% Classes and languages.
\def\FREACH{\text{\rm AFFINEinSL}}
\def\EQUAL{\text{\rm EQUAL}}
\def\COPY{\text{\rm COPY}}
\def\lang{\mathcal{L}}
\def\LDPA{\lang_{\text{\rm DetPA}}}
\def\LPA{\lang_{\text{\rm PA}}}
\def\LBPA{\lang_{\text{\rm BoundedPA}}}
\def\LBDPA{\lang_{\text{\rm BoundedDetPA}}}
\def\LDAPA{\lang_{\text{\rm DetAPA}}}
\def\LAPA{\lang_{\text{\rm APA}}}
\def\LDAPAM{\lang_{\text{\rm DetAPA-FM}}}
\def\LAPAM{\lang_{\text{\rm APA-FM}}}
\def\LDCA{\lang_{\text{\rm DetCA}}}
\def\LCA{\lang_{\text{\rm CA}}}
\def\LLPA{\lang_{\text{\rm LPA}}}
\def\LDLPA{\lang_{\text{\rm DetLPA}}}
\def\LSCA{\lang_{\text{\rm SCA}}}
\def\LRBCM{\lang_{\text{\rm RBCM}}}
\def\LDRBCM{\lang_{\text{\rm DetRBCM}}}
\def\BSL{{\rm BSL}}
\def\BDD{{\rm BOUNDED}}
\def\CSL{{\rm CSL}}
\def\REG{{\rm REG}}
\def\CFL{{\rm CFL}}
\def\NSPACE{{\rm NSPACE}}

%% Draft and non-draft.
\newif\ifdraft
\def\drafton{\global\drafttrue%
  \global\adrafttrue%
  \setlength\overfullrule{5pt}}
\def\draftoff{\global\draftfalse%
  \global\adraftfalse%
  \setlength\overfullrule{0pt}}
\draftoff

%% Tweak of eptcs class.
\def\switchtoinstitutes{\end{tabular}\\\begin{tabular}[t]{c}}

%% Array displayed.
\newenvironment{disarray}%
{\everymath{\smallskip\displaystyle\everymath{}}\array}%
{\endarray}

%% Automata in Tikz.
\newenvironment{automaton}[1][]{
  \begin{center}
    \begin{tikzpicture}[shorten >=1pt,initial text=,
      line width=.65pt,
      state/.append style={minimum size=1.65em},
      every state/.style={fill=white},
      node distance=2cm,%
      smallstate/.style={state,minimum size=1em,inner sep=0pt},on grid,auto,#1]}
    {\end{tikzpicture}
  \end{center}%\vspace{-\baselineskip}
}

\def\bar#1{\overline{#1}}


%% Theorems and definitions, and such.
\newcounter{defc}
\newtheorem{theorem}{\textbf{Theorem}}
\newtheorem{lemma}[theorem]{\textbf{Lemma}}
\newtheorem{corollary}[theorem]{\textbf{Corollary}}
\newtheorem{proposition}[theorem]{\textbf{Proposition}}
\newtheorem{fact}[theorem]{\textbf{Fact}}
\newtheorem*{claim*}{\textbf{Claim}}
\theoremstyle{definition}
\newtheorem{definition}[defc]{\textbf{Definition}}

\makeatother


==> eptcsdata.tex <==
\providecommand{\firstpage}{93}
\providecommand{\publicationstatus}{P. Ambro{\v z}, {\v S}. Holub and Z. Mas\'akov\'a (Eds.):\\
8th International Conference WORDS 2011\\
EPTCS 63, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.63.13}{10.4204/EPTCS.63.13}}
\pdfoutput=1

